Sonus Texere! Automated Dense Soundtrack Construction for Books using Movie Adaptations

Reading, much like music listening, is an immersive experience that transports readers while taking them on an emotional journey. Listening to complementary music has the potential to amplify the reading experience, especially when the music is stylistically cohesive and emotionally relevant. In this paper, we propose the first fully automatic method to build a dense soundtrack for books, which can play high-quality instrumental music for the entirety of the reading duration. Our work employs a unique text processing and music weaving pipeline that determines the context and emotional composition of scenes in a chapter. This allows our method to identify and play relevant excerpts from the soundtrack of the book's movie adaptation. By relying on the movie composer's craftsmanship, our book soundtracks include expert-made motifs and other scene-specific musical characteristics. We validate the design decisions of our approach through a perceptual study. Our readers note that the book soundtrack greatly enhanced their reading experience, due to high immersiveness granted via uninterrupted and style-consistent music, and a heightened emotional state attained via high precision emotion and scene context recognition.

==> ISMIR2022_lbd.tex <==






















==> conf_meta.tex <==






































==> header.tex <==
\makeatletter
\let\@oldmaketitle\@maketitle
\renewcommand{\@maketitle}{\@oldmaketitle
\vspace{0.2cm}
\centering
\includegraphics[width=0.6\linewidth]{figs/placeholder_header.png}\\
\captionof{figure}{Hello this is the header image, and this is the caption \jaidev{Fix this figure - needs numbering, caption position is sus}}
\label{fig:header_img}
\vspace{0.4cm}
}

==> planning.tex <==









    
    


    
    
    
    
    
    
    



==> sections/3_approach.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/placeholder_header.png}
    \caption{Overview of approach}
    \label{fig:approach_overview}
\end{figure*}

\section{Our Approach}

\subsection{General Overview}

A key problem with building a soundtrack for books is the sheer scale of components. A typical book can take many hours to read, which must also be matched by its soundtrack. Within the book itself, there are multiple chapters, with each having distinct sections marked by a certain theme, emotion, or location. An ideal soundtrack should respect these scene boundaries and change accordingly. 

Since we focus on adapting the movie soundtrack, we face scale issues at the movie and soundtrack level as well. Movies do not come with predefined scene breaks or context information that can simplify movie processing. On the music side, while we do have different songs from the soundtrack that are largely locally homogenous/consistent, they are rarely played in its entirety, at a stretch, in the movie. Composers typically segment the song into pieces and play these at opportune moments to maximise \green{emotional payoffs}. A song that we obtain via the soundtrack album is hence, a reflection of an entire narrative arc and cannot be played for shorter sections of the same.
Our method resolves these issues by first breaking each modality (movie, book, and music) into manageable segments. We then approach the soundtrack construction process as a multi-modal retrieval task (Figure \ref{fig:approach_overview}), where for every book segment, we fetch a corresponding music segment, based on cues present in a relevant movie segment. 

\blue{In this section, we begin with text segmentation (Sec \ref{text_segmentation}), which defines the content to soundtrack}. We then discuss how we align the book and movie (Sec \ref{text_movie}) to provide narrative context and obtain musical clues about the soundtrack played at that plot point. Finally, we align the book and music (Sec \ref{book_movie}) using these cues to build the soundtrack.

\subsection{Text Segmentation}
\label{text_segmentation}

Text scene segmentation is the problem of finding boundaries in text that divide narratives, based on its theme, location, activity composition, character constellation, or even time \cite{Zehe2021DetectingSI}. Due to the absence of large datasets for this task, we adopt an unsupervised approach, temporally weighted hierarchical clustering \cite{sarfraz2021temporally}. Here, we encode each paragraph of a chapter using a pretrained MPNet language model \cite{song2020mpnet} and cluster spatially and semantically similar paragraphs into one segment. We also considered TextTiling \cite{Hearst1997TextTS} and TopicTiling \cite{Riedl_topictil} for the same but obtained inferior results. TextTiling \cite{Hearst1997TextTS} tended to uniformly partition chapters while TopicTiling \cite{Riedl_topictil} often resulted in hypersegmentation. We find that hierarchical clustering yielded segments that largely respected narrative shifts, even though it lacked consistency in the differentiating factor used (characters/theme/location). 

% The subjectivity of each factor makes this highly challenging and the absence of large datasets for this task makes supervised approaches difficult, with prior work \cite{Kurfali2021BreakingTN, Gombert2021TwinBC} struggling to achieve high accuracies.


\subsection{Text-Movie Alignment}
\label{text_movie}

\subsubsection{Movie-Scene Detection}
We segment the movie into scenes using the approach described in \cite{tapaswi_storygraph}. It breaks the movie into short segments (shots) and uses dynamic programming to find scene boundaries (a scene consists of multiple shots), while optimising for maximum intra-scene shot similarity. 

\subsubsection{Chapter-Scene Alignment}
With the obtained movie scenes, we perform a coarse chapter-level book to movie alignment, where each chapter is assigned a set of scenes from the movie. Here, we use an approach similar to \cite{TapaswiB2M} where similarities in character histograms and dialogues are used with a Dynamic Time Warping algorithm to align chapters and scenes.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{figs/placeholder_header.png}
    \caption{Keystrength based segmentation -> Sim Matrix -> Novelty}
    \label{fig:music_segment}
\end{figure*}
 
\subsubsection{Paragraph-Scene Refinement}

The coarse alignment obtained earlier cannot directly be used for soundtracking as a chapter contains distinct segments that likely need different music. Therefore, we refine our alignment to a text segment-scene level by using dialogue matches - scenes with similar dialogues are assigned to a unique text segment. As this only accounts for a small fraction of segments, we additionally resort to zero-shot chunk-scene alignment. Specifically, we use the vision-language model CLIP \cite{radford2021learning} to match frames in the movie with chunk sentences, based on similarity in their shared embedding space.

Since a text segment contains many sentences, including dialogues and mundane details, we attempt to prune this set to only consider important sentences that are likely visually represented. First, we use a TF-IDF based scoring system to rank all sentences, as rare characters or items are more likely to give confident matches than recurring/regular characters/objects. Then, we only keep those sentences that can be visually represented, using the word concreteness index \cite{Brysbaert2014ConcretenessRF} which measures how likely a word can be seen or experienced. Finally, we take the top remaining sentences and encode them with CLIP and calculate cosine similarity with all CLIP embedded shots in the chapter's scenes (Figure \ref{fig:clip}). For those with a high score, we assign the scene to the corresponding text segment.

\begin{figure}[b!]
    \centering
    \includegraphics[width=\linewidth]{figs/placeholder_square.png}
    \caption{Examples of CLIP-based paragraph-scene alignment.}
    \label{fig:clip}
\end{figure}

\subsection{Book-Music Alignment}
\label{book_movie}

\subsubsection{Movie Based Retrieval}

With the final book-movie alignment in hand, we focus on identifying the music in each movie scene use the alignment to play the same track for the corresponding text segment. We accomplish this using Shazam \footnote{https://www.shazam.com/}, a well-established audio-fingerprint based search application. By passing the entire movie's audio through the Shazam API, we obtain a high-precision guess for the music played at any scene, which we then assign to that text segment. In principle, any audio fingerprinting approach should work, but we found that Shazam was the most accurate in the presence of background noise and dialogues.

% - Audio fingerprinting based approach
% - We found that it did well even in the presence of noise / dialogue
% - Used shazam, in principle an audio fingerprinting thing can work, just needs to be robust
% \glipsum{1}

\subsubsection{Music Segmentation}

% (\textit{Howard Shore's} Lord of the Rings' Prologue is 7 minutes long and tells the entire story of the ring,

The movie based retrieval approach can often result in text segments being assigned long tracks, for otherwise short narratives. This is unlike movies, where only a portion of the track plays, with the entire track representing a long narrative arc. Hence, we focus on creating homogenous emotionally-cohesive track segments from these that can be played continuously for a single text segment. Once the track is segmented, we choose an emotionally relevant one, using the procedure described in section \ref{emotion_retr}.

A key feature that the segments are required to reflect are emotions intended to be conveyed by the director/composer. Since we expect homogeneity in emotion for music segments, keystrength can serve as a good attribute as it captures the tonal properties of music, and tonal changes likely suggest emotional shifts (e.g: major to minor suggesting a shift from positive to negative valence). Keystrength is an acoustic feature that gives us a probability for each possible key resulting in a 24 dimensional vector (12 major and 12 minor keys). We use a window size of 10 seconds with an 85\% overlap, which helps ignore minor local variations in the track while retaining larger shifts. We then compute a self-similarity matrix \cite{Foote2003MediaSU} of the time-varying keystrength vector which is used to subsequently to calculate the novelty curve with a kernel size of 64 \cite{Foote2003MediaSU}. The peaks in the novelty curve determine points of change. Finally, we use those peaks as our segment boundaries.

% Tracks in an original soundtrack are typically quite long, even though their appearance in the movie is much shorter. When compared to such movies, books move at a much slower pace and when a long track is played, it can lose relevance beyond a certain point, especially if there is an emotional or plot shift midway. Hence, this requires us to create homogeneous chunks that can be played continuously for a single text segment with the option of looping if the text segment is shorter than the music segment.


% We first calculate the keystrength of track segments \cite{Gmez2006TonalDO} which gives us a probability for each possible key of the song at various instants. We use a window size of 10 seconds with an 85 \% overlap, which helps ignore minor local variations in the track while retaining larger shifts. We opt for keystrength as it is a good representation of the tonal properties of the track. Since we expect homogeneity in emotion for music segments, keystrength can serve as a good attribute as it captures the tonal properties of music and tonal changes can likely suggest emotional shifts.

% Using keystrength, we compute a self-similarity matrix \cite{Foote2003MediaSU}, which can help visualise locally similar regions and potential segment boundaries. Finally, we compute the novelty curve over this matrix \cite{Foote2003MediaSU} to automatically determine points of significant change. We use a kernel size of 64 here to smooth the curve and only consider significant shits. Finally, we use peaks from this that are sufficiently spaced apart as our segment boundaries. Note that we loop these segments when reading a particular text chunk, due to which we prefer segments that are at least 30 seconds long, below which the music would be too highly periodic.

% we merge it with another segment. 

% This process can be seen in figure \ref{fig:music_segment}.
 
\subsubsection{Emotion Based Retrieval}
\label{emotion_retr}

The fingerprinting based approach results in a sparse soundtrack as some movie scenes have no music or had music that could not be identified. Even for those scenes with a matched track, we are only interested in a few segments that match the corresponding text's emotion. Here, we rely on the emotional composition of the text segment to resolve these issues by finding a music segment that is similar. For text, we classify each paragraph into positive, neutral, or negative emotions using a BERT based emotion classifier \cite{demszky2020goemotions}, trained on Reddit comments. The emotion of a text-segment is then considered to be the majority across all paragraphs. For music, we calculate valence based on the mode of the song (major or minor), as tracks in minor tend to be associated with negative emotions and tracks in major are perceived as brighter and joyous. With these text/music emotion labels, we can finally align the two using the aforementioned movie retrieval technique or randomly fetch an emotionally similar segment.

% Once these steps, summarised in figure \ref{fig:approach_overview}, are complete, we obtain short musical pieces for each text segment, which can then be played using an application, like one mentioned in section \ref{reading_app}.

% - There are some movie sections where no music is played or where no music could be identified
% - RMS and mode used

% \glipsum{1}
